On Designing Modulation for Over-the-Air Computation -- Part I: Noise-Aware Design

Over-the-air computation (OAC) leverages the physical superposition property of wireless multiple access channels (MACs) to compute functions while communication occurs, enabling scalable and low-latency processing in distributed networks. While analog OAC methods suffer from noise sensitivity and hardware constraints, existing digital approaches are often limited in design complexity, which may hinder scalability and fail to exploit spectral efficiency fully. This two-part paper revisits and extends the ChannelComp framework, a general methodology for computing arbitrary finite-valued functions using digital modulation. In Part I, we develop a novel constellation design approach that is aware of the noise distribution and formulates the encoder design as a max-min optimization problem using noise-tailored distance metrics. Our design supports noise models, including Gaussian, Laplace, and heavy-tailed distributions. We further demonstrate that, for heavy-tailed noise, the optimal ChannelComp setup coincides with the solution to the corresponding max-min criterion for the channel noise with heavy-tailed distributions. Numerical experiments confirm that our noise-aware design achieves a substantially lower mean-square error than leading digital OAC methods over noisy MACs. In Part II, we consider a constellation design with a quantization-based sampling scheme to enhance modulation scalability and computational accuracy for large-scale digital OAC.

==> acronyms.tex <==
\begin{acronym}[LTE-Advanced]%\addtolength{\itemsep}{-0.5\baselineskip}
  \acro{2G}{second generation}
  \acro{ASK}{amplitude-shift keying}
  \acro{SumComp}{sum computation}
  \acro{6G}{sixth generation}
  \acro{3-DAP}{3-dimensional assignment problem}
  \acro{AA}{antenna array}
  \acro{AC}{admission control}
  \acro{AD}{attack-decay}
  \acro{ADC}{analog-to-digital conversion}
  \acro{ADMM}{alternating direction method of multipliers}
  \acro{ADSL}{asymmetric digital subscriber line}
  \acro{AHW}{alternate hop-and-wait}
  \acro{AI}{artificial intelligence}
  \acro{AirComp}{over-the-air computation}
  \acro{AM}{amplitude modulation}
  \acro{AMC}{adaptive modulation and coding}
  \acro{AP}{\LU{A}{a}ccess \LU{P}{p}oint}
  \acro{APA}{adaptive power allocation}
  \acro{ARMA}{autoregressive moving average}
  \acro{ARQ}{\LU{A}{a}utomatic \LU{R}{r}epeat \LU{R}{r}equest}
  \acro{ATES}{adaptive throughput-based efficiency-satisfaction trade-off}
  \acro{AWGN}{additive white Gaussian noise}
  \acro{BAA}{\LU{B}{b}roadband \LU{A}{a}nalog \LU{A}{a}ggregation}
  \acro{BB}{branch and bound}
  \acro{BCD}{block coordinate descent}
  \acro{BD}{block diagonalization}
  \acro{BER}{bit error rate}
  \acro{BF}{best fit}
  \acro{BFD}{bidirectional full duplex}
  \acro{BLER}{bLock error rate}
  \acro{BPC}{binary power control}
  \acro{BPSK}{binary phase-shift keying}
  \acro{BRA}{balanced random allocation}
  \acro{BS}{base station}
  \acro{BSUM}{block successive upper-bound minimization}
  \acro{CAP}{combinatorial allocation problem}
  \acro{CAPEX}{capital expenditure}
  \acro{CBF}{coordinated beamforming}
  \acro{CBR}{constant bit rate}
  \acro{CBS}{class based scheduling}
  \acro{CC}{congestion control}
  \acro{CDF}{cumulative distribution function}
  \acro{CDMA}{code-division multiple access}
  \acro{CE}{\LU{C}{c}hannel \LU{E}{e}stimation}
  \acro{CL}{closed loop}
  \acro{CLPC}{closed loop power control}
  \acro{CML}{centralized machine learning}
  \acro{CNR}{channel-to-noise ratio}
  \acro{CNN}{\LU{C}{c}onvolutional \LU{N}{n}eural \LU{N}{n}etwork}
  \acro{CP}{computation point}
  \acro{CPA}{cellular protection algorithm}
  \acro{CPICH}{common pilot channel}
  \acro{CoCoA}{\LU{C}{c}ommunication efficient distributed dual \LU{C}{c}oordinate \LU{A}{a}scent}
  \acro{CoMAC}{\LU{C}{c}omputation over \LU{M}{m}ultiple-\LU{A}{a}ccess \LU{C}{c}hannels}
  \acro{CoMP}{coordinated multi-point}
  \acro{CQI}{channel quality indicator}
  \acro{CRM}{constrained rate maximization}
  \acro{CRN}{cognitive radio network}
  \acro{CS}{coordinated scheduling}
  \acro{CSI}{\LU{C}{c}hannel \LU{S}{s}tate \LU{I}{i}nformation}
  \acro{CSMA}{\LU{C}{c}arrier \LU{S}{s}ense \LU{M}{m}ultiple \LU{A}{a}ccess}
  \acro{CUE}{cellular user equipment}
  \acro{D2D}{device-to-device}
  \acro{DAC}{digital-to-analog converter}
  \acro{DC}{direct current}
  \acro{DCA}{dynamic channel allocation}
  \acro{DE}{differential evolution}
  \acro{DFT}{discrete Fourier transform}
  \acro{DIST}{distance}
  \acro{DL}{downlink}
  \acro{DMA}{double moving average}
  \acro{DML}{distributed machine learning}
  \acro{DMRS}{demodulation reference signal}
  \acro{D2DM}{D2D mode}
  \acro{DMS}{D2D mode selection}
  \acro{DNN}{deep neural network}
  \acro{DPC}{dirty paper coding}
  \acro{DRA}{dynamic resource assignment}
  \acro{DSA}{dynamic spectrum access}
  \acro{DSGD}{\LU{D}{d}istributed \LU{S}{s}tochastic \LU{G}{g}radient \LU{D}{d}escent}
  \acro{DSM}{delay-based satisfaction maximization}
  \acro{ECC}{electronic communications committee}
  \acro{EFLC}{error feedback based load control}
  \acro{EI}{efficiency indicator}
  \acro{eNB}{evolved Node B}
  \acro{EPA}{equal power allocation}
  \acro{EPC}{evolved packet core}
  \acro{EPS}{evolved packet system}
  \acro{E-UTRAN}{evolved universal terrestrial radio access network}
  \acro{ES}{edge server}
  \acro{FC}{\LU{F}{f}usion \LU{C}{c}enter}
  \acro{FSK}{frequency-shift keying}
  \acro{FD}{\LU{F}{f}ederated \LU{D}{d}istillation}
  \acro{FDD}{frequency division duplex}
  \acro{FDM}{frequency division multiplexing}
  \acro{FDMA}{\LU{F}{f}requency \LU{D}{d}ivision \LU{M}{m}ultiple \LU{A}{a}ccess}
  \acro{FedAvg}{\LU{F}{f}ederated \LU{A}{a}veraging}
  \acro{FER}{frame erasure rate}
  \acro{FF}{fast fading}
  \acro{FL}{federated learning}
  \acro{FSB}{fixed switched beamforming}
  \acro{FST}{fixed SNR target}
  \acro{FTP}{file transfer protocol}
  \acro{GA}{genetic algorithm}
  \acro{GBR}{guaranteed bit rate}
  \acro{GD}{gradient descent}
  \acro{GLR}{gain to leakage ratio}
  \acro{GOS}{generated orthogonal sequence}
  \acro{GPL}{GNU general public license}
  \acro{GRP}{grouping}
  \acro{HARQ}{hybrid automatic repeat request}
  \acro{HD}{half-duplex}
  \acro{HMS}{harmonic mode selection}
  \acro{HOL}{head of line}
  \acro{HSDPA}{high-speed downlink packet access}
  \acro{HSPA}{high speed packet access}
  \acro{HTTP}{hypertext transfer protocol}
  \acro{ICMP}{internet control message protocol}
  \acro{ICI}{intercell interference}
  \acro{ID}{identification}
  \acro{IETF}{internet engineering task force}
  \acro{ILP}{integer linear program}
  \acro{JRAPAP}{joint RB assignment and power allocation problem}
  \acro{UID}{unique identification}
  \acro{IID}{\LU{I}{i}ndependent and \LU{I}{i}dentically \LU{D}{d}istributed}
  \acro{IIR}{infinite impulse response}
  \acro{ILP}{integer linear problem}
  \acro{IMT}{international mobile telecommunications}
  \acro{INV}{inverted norm-based grouping}
  \acro{IoT}{internet of things}
  \acro{IP}{integer programming}
  \acro{IPv6}{internet protocol version 6}
  \acro{IQ}{in-phase quadrature}
  \acro{ISD}{inter-site distance}
  \acro{ISI}{inter symbol interference}
  \acro{ITU}{international telecommunication union}
  \acro{JAFM}{joint assignment and fairness maximization}
  \acro{JAFMA}{joint assignment and fairness maximization algorithm}
  \acro{JOAS}{joint opportunistic assignment and scheduling}
  \acro{JOS}{joint opportunistic scheduling}
  \acro{JP}{joint processing}
	\acro{JS}{jump-stay}
  \acro{KKT}{Karush-Kuhn-Tucker}
  \acro{L3}{Layer-3}
  \acro{LAC}{link admission control}
  \acro{LA}{link adaptation}
  \acro{LC}{load control}
  \acro{LDC}{\LU{L}{l}earning-\LU{D}{d}riven \LU{C}{c}ommunication}
  \acro{LOS}{line of sight}
  \acro{LP}{linear programming}
  \acro{LTE}{long term evolution}
	\acro{LTE-A}{\ac{LTE}-advanced}
  \acro{LTE-Advanced}{long term evolution advanced}
  \acro{M2M}{machine-to-machine}
  \acro{MAC}{multiple access channel}
  \acro{MANET}{mobile ad hoc network}
  \acro{MC}{modular clock}
  \acro{MCS}{modulation and coding scheme}
  \acro{MDB}{measured delay based}
  \acro{MDI}{minimum D2D interference}
  \acro{MF}{matched filter}
  \acro{MG}{maximum gain}
  \acro{MH}{multi-hop}
  \acro{MIMO}{\LU{M}{m}ultiple \LU{I}{i}nput \LU{M}{m}ultiple \LU{O}{o}utput}
  \acro{MINLP}{mixed integer nonlinear programming}
  \acro{MIP}{mixed integer programming}
  \acro{MISO}{multiple input single output}
  \acro{ML}{machine learning}
  \acro{MLWDF}{modified largest weighted delay first}
  \acro{MME}{mobility management entity}
  \acro{MMSE}{minimum mean squared error}
  \acro{MOS}{mean opinion score}
  \acro{MPF}{multicarrier proportional fair}
  \acro{MRA}{maximum rate allocation}
  \acro{MR}{maximum rate}
  \acro{MRC}{maximum ratio combining}
  \acro{MRT}{maximum ratio transmission}
  \acro{MRUS}{maximum rate with user satisfaction}
  \acro{MS}{mode selection}
  \acro{MAE}{\LU{M}{m}ean \LU{A}{a}bsolute \LU{E}{e}rror}
  \acro{MSE}{\LU{M}{m}ean \LU{S}{s}quared \LU{E}{e}rror}
  \acro{MSI}{multi-stream interference}
  \acro{MTC}{machine-type communication}
  \acro{MTSI}{multimedia telephony services over IMS}
  \acro{MTSM}{modified throughput-based satisfaction maximization}
  \acro{MU-MIMO}{multi-user multiple input multiple output}
  \acro{MU}{multi-user}
  \acro{NAS}{non-access stratum}
  \acro{NB}{Node B}
  \acro{NCL}{neighbor cell list}
  \acro{NLP}{nonlinear programming}
  \acro{NLOS}{non-line of sight}
  \acro{NMSE}{normalized mean square error}
  \acro{NN}{neural network}
  \acro{NOMA}{\LU{N}{n}on-\LU{O}{o}rthogonal \LU{M}{m}ultiple \LU{A}{a}ccess}
  \acro{NORM}{normalized projection-based grouping}
  \acro{NP}{non-polynomial time}
  \acro{NRT}{non-real time}
  \acro{NSPS}{national security and public safety services}
  \acro{O2I}{outdoor to indoor}
  \acro{OAC}{over-the-air computation}
  \acro{OFDMA}{\LU{O}{o}rthogonal \LU{F}{f}requency \LU{D}{d}ivision \LU{M}{m}ultiple \LU{A}{a}ccess}
  \acro{OFDM}{orthogonal frequency division multiplexing}
  \acro{OFPC}{open loop with fractional path loss compensation}
	\acro{O2I}{outdoor-to-indoor}
  \acro{OL}{open loop}
  \acro{OLPC}{open-loop power control}
  \acro{OL-PC}{open-loop power control}
  \acro{OPEX}{operational expenditure}
  \acro{ORB}{orthogonal random beamforming}
  \acro{JO-PF}{joint opportunistic proportional fair}
  \acro{OSI}{open systems interconnection}
  \acro{PM}{phase modulation}
  \acro{PAM}{pulse-amplitude modulation}
  \acro{PAIR}{D2D pair gain-based grouping}
  \acro{PAPR}{peak-to-average power ratio}
  \acro{P2P}{peer-to-peer}
  \acro{PC}{power control}
  \acro{PCI}{physical cell ID}
  \acro{PDCCH}{physical downlink control channel}
  \acro{PDD}{penalty dual decomposition}
  \acro{PDF}{probability density function}
  \acro{PER}{packet error rate}
  \acro{PF}{proportional fair}
  \acro{P-GW}{packet data network gateway}
  \acro{PL}{pathloss}
  \acro{PLL}{phase-locked loop}
  \acro{PRB}{physical resource block}
  \acro{PROJ}{projection-based grouping}
  \acro{ProSe}{proximity services}
  \acro{PS}{\LU{P}{p}arameter \LU{S}{s}erver}
  \acro{PSO}{particle swarm optimization}
  \acro{PUCCH}{physical uplink control channel}
  \acro{PZF}{projected zero-forcing}
  \acro{QAM}{quadrature amplitude modulation}
  \acro{QoS}{quality of service}
  \acro{QPSK}{quadrature-phase shift keying}
  \acro{RAISES}{reallocation-based assignment for improved spectral efficiency and satisfaction}
  \acro{RAN}{radio access network}
  \acro{RA}{resource allocation}
  \acro{RAT}{radio access technology}
  \acro{RATE}{rate-based}
  \acro{RB}{resource block}
  \acro{RBG}{resource block group}
  \acro{REF}{reference grouping}
  \acro{RF}{radio frequency}
  \acro{RLC}{radio link control}
  \acro{RM}{rate maximization}
  \acro{RNC}{radio network controller}
  \acro{RND}{random grouping}
  \acro{RRA}{radio resource allocation}
  \acro{RRM}{\LU{R}{r}adio \LU{R}{r}esource \LU{M}{m}anagement}
  \acro{RSCP}{received signal code power}
  \acro{RSRP}{reference signal receive power}
  \acro{RSRQ}{reference signal receive quality}
  \acro{RR}{round robin}
  \acro{RRC}{radio resource control}
  \acro{RSSI}{received signal strength indicator}
  \acro{RT}{real time}
  \acro{RU}{resource unit}
  \acro{RUNE}{rudimentary network emulator}
  \acro{RV}{random variable}
  \acro{SAC}{session admission control}
  \acro{SCM}{spatial channel model}
  \acro{SC-FDMA}{single carrier - frequency division multiple access}
  \acro{SD}{soft dropping}
  \acro{S-D}{source-destination}
  \acro{SDPC}{soft dropping power control}
  \acro{SDMA}{space-division multiple access}
  \acro{SDR}{semidefinite relaxation}
  \acro{SDP}{semidefinite programming}
  \acro{SER}{symbol error rate}
  \acro{SES}{simple exponential smoothing}
  \acro{S-GW}{serving gateway}
  \acro{SGD}{\LU{S}{s}tochastic \LU{G}{g}radient \LU{D}{d}escent}  
  \acro{SINR}{signal-to-interference-plus-noise ratio}
  \acro{SI}{self-interference}
  \acro{SIP}{Session Initiation Protocol}
  \acro{SISO}{\LU{S}{s}ingle \LU{I}{i}nput \LU{S}{s}ingle \LU{O}{o}utput}
  \acro{SIMO}{Single Input Multiple Output}
  \acro{SIR}{signal to interference ratio}
  \acro{SLNR}{Signal-to-Leakage-plus-Noise Ratio}
  \acro{SMA}{simple moving average}
  \acro{SNR}{\LU{S}{s}ignal-to-\LU{N}{n}oise \LU{R}{r}atio}
  \acro{SORA}{satisfaction oriented resource allocation}
  \acro{SORA-NRT}{satisfaction-oriented resource allocation for non-real time services}
  \acro{SORA-RT}{satisfaction-oriented resource allocation for real time services}
  \acro{SPF}{single-carrier proportional fair}
  \acro{SRA}{sequential removal algorithm}
  \acro{SRS}{sounding reference signal}
  \acro{SU-MIMO}{single-user multiple input multiple output}
  \acro{SU}{single-user}
  \acro{SVD}{singular value decomposition}
  \acro{SVM}{\LU{S}{s}upport \LU{V}{v}ector \LU{M}{m}achine}
  \acro{TCP}{Transmission Control Protocol}
  \acro{TDD}{time division duplex}
  \acro{TDMA}{\LU{T}{t}ime \LU{D}{d}ivision \LU{M}{m}ultiple \LU{A}{a}ccess}
  \acro{TNFD}{three node full duplex}
  \acro{TETRA}{terrestrial trunked radio}
  \acro{TP}{transmit power}
  \acro{TPC}{transmit power control}
  \acro{TTI}{transmission time interval}
  \acro{TTR}{time-to-rendezvous}
  \acro{TSM}{throughput-based satisfaction maximization}
  \acro{TU}{typical urban}
  \acro{UE}{\LU{U}{u}ser \LU{E}{e}quipment}
  \acro{UEPS}{urgency and efficiency-based packet scheduling}
  \acro{UL}{uplink}
  \acro{UMTS}{universal mobile telecommunications system}
  \acro{URI}{uniform resource identifier}
  \acro{URM}{unconstrained rate maximization}
  \acro{VR}{virtual resource}
  \acro{VoIP}{voice over IP}
  \acro{WAN}{wireless access network}
  \acro{WCDMA}{wideband code division multiple access}
  \acro{WF}{water-filling}
  \acro{WiMAX}{worldwide interoperability for microwave access}
  \acro{WINNER}{wireless world initiative new radio}
  \acro{WLAN}{wireless local area network}
  \acro{WMMSE}{weighted minimum mean square error}
  \acro{WMPF}{weighted multicarrier proportional fair}
  \acro{WPF}{weighted proportional fair}
  \acro{WSN}{wireless sensor network}
  \acro{WWW}{world wide web}
  \acro{XIXO}{(single or multiple) input (single or multiple) output}
  \acro{ZF}{zero-forcing}
  \acro{ZMCSCG}{zero mean circularly symmetric complex Gaussian}
\end{acronym}

